S2ST: Image-to-Image Translation in the Seed Space of Latent Diffusion

Image-to-image translation (I2IT) refers to the process of transforming images from a source domain to a target domain while maintaining a fundamental connection in terms of image content. In the past few years, remarkable advancements in I2IT were achieved by Generative Adversarial Networks (GANs), which nevertheless struggle with translations requiring high precision. Recently, Diffusion Models have established themselves as the engine of choice for image generation. In this paper we introduce S2ST, a novel framework designed to accomplish global I2IT in complex photorealistic images, such as day-to-night or clear-to-rain translations of automotive scenes. S2ST operates within the seed space of a Latent Diffusion Model, thereby leveraging the powerful image priors learned by the latter. We show that S2ST surpasses state-of-the-art GAN-based I2IT methods, as well as diffusion-based approaches, for complex automotive scenes, improving fidelity while respecting the target domain's appearance across a variety of domains. Notably, S2ST obviates the necessity for training domain-specific translation networks.

==> sec/1_1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Image-to-Image Translation (I2IT) refers to the process of converting an image from one domain to another while preserving its content and structure. Unpaired Image-to-Image Translation (Unpaired I2IT) is a noteworthy subset, focused on translating images without requiring pairs of source and target images for training and validation. Despite the remarkable advancements I2IT facilitated by Generative Adversarial Networks (GANs) in recent years (e.g., \cite{zhu2017unpaired, liu2017unsupervised,  huang2018multimodal, jiang2020tsit, dutta2022seeing}) there has been a noticeable {\color{purple} slowdown} in progress during the past few years. 
\dani{I would not necessarily claim a slowdown - people have turned to diffusion, so naturally fewer attempts were made to advance and improve GAN-based solution. It is safer to just point out the limitations that exist in SoTA GAN-based methods, as done below. Perhaps a more balanced statement could point out that some translations are done very well with GANs, while some are not.}
Even state-of-the-art (SoTA) GAN-based I2IT models encounter  challenges related to: (i) accurately synthesizing photo-realistic images in the target domain's manifold and (ii) handling multi-domain translation, as current GANs are typically limited to learning a specific mappings from one source to one target. 

In recent years, text-to-image diffusion models like DALL-E2 \cite{ramesh2022hierarchical}, Imagen \cite{saharia2022photorealistic}, and Stable Diffusion \cite{rombach2022high}, have demonstrated impressive capabilities in generating text-guided photo-realistic and diverse synthetic images from random noises. \edit{In this paper we use the term \textbf{seed space} to denote the infinite set of random samples (seeds) from a high-dimensional space that initiates the difussion process \cite{samuel2023norm}.}  Previous works have harnessed the potent generative engine inherent in diffusion models for advanced image editing tasks. While these papers have indeed showcased impressive results, the primary emphasis in most of them has centered on localized editing of relatively simple, object-centered images.
\dani{This claim can also be controversial. In the past year there have been so many works on image editing with diffusion, many of them are non-local and applicable to complex scenes. I think a better point to make migt be that diffusion-based edits typically change the content in a manner that can be difficult to control.}

To address the aforementioned challenges, we propose Seed-to-Seed Translation ($S2ST$), a diffusion-based I2IT solution that harnesses the potent generative engine of a trained diffusion model to perform global edits (e.g., day-to-night, clear-to-foggy etc.) within complex (automotive) scenes. We show that $S2ST$ outperforms state-of-the-art GAN-based methods in term of it's capacity to learn the target domain's appearance across diverse domains, while eliminating the need for training domain-specific networks.
\dani{I think we should position the approach as primarily designed for the types of translations that we demonstrate, claim that they are challenging and/or have relatively unique requirements, and we propose a method that is well-suited for them. If we make it sound like a general I2I method, we will be expected to evaluate and compare also on other types of I2I translations...}

To achieve such editability, as well as fidelity to the source content, We do a simple 3-steps process, as depicted in \Cref{fig:overall}, with Stable Diffusion \cite{rombach2022high} as the generative engine: We first invert the source image to the seed-space using $\DDIM_\mathrm{inversion}$ (denoted $\DDIM_\mathrm{inv}$) \cite{song2020denoising}. 
\dani{Was the term seed-space coined in some previous work? If yes, we should cite, if not we should exlpain/define what it is}
Then, we translate the source-related seed within the seed space to an optimized seed, correlated with the target domain, while enforcing structural similarity between the source and the target latents. Finally, we use the two trajectories defined by the $\DDIM_\mathrm{inv}$  and $\DDIM_\mathrm{sampling}$  (denoted $\DDIM_\mathrm{sam}$, from the optimized-seed to the ``clean'' latent domain) to further enhance the structural similarity between the source image and the translated one.

With a text descriptor describing the target domain, and a few ($\sim5$) images from the target domain, our approach can generate a synthetic image that is well-aligned with the target domain while keeping the structure and content of the source image. Using both quantitative and qualitative metrics we show that our method outperforms SoTA GAN-based I2IT and other Diffusion based Image-Editing methods in terms of photo-realism and content preservation.

%We summarize our main contributions as follows:
%\begin{enumerate}
%    \item We present $S2ST$, the first diffusion-based I2IT technique that allows a global editing of complex scenes.
%    \item We suggest a correlation factor between the different source-to-target translation and the different channels of Stable Diffusion's latent space to allow semi-disentanglement between "structure" and "appearance" in the translation process.
%\end{enumerate}
For additional results and access to the accompanying code, please visit our project-page at {\color{purple}$[URL]$}.

\begin{figure}[t]
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{figures/overall.png}

   \caption{\textbf{S2ST overall framework:} The input image is being inverted to the seed space, where it is translated to the target domain. Finally, a Trajectory Optimization phase is being performed to enhance structural similarity between the source image and the translated one.}
   \label{fig:overall}
\end{figure}
%-------------------------------------------------------------------------
%-----------------------------          ----------------------------------
%-----------------------------UNTIL HERE----------------------------------
%-----------------------------          ----------------------------------
%-------------------------------------------------------------------------
\newif\ifshowparagraph % Define a new conditional
\ifshowparagraph

\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}
\fi

==> sec/2_2_related.tex <==
\section{Related Work}
\label{sec:RelatedWork}

Unpaired I2IT has garnered increasing attention and made significant progress in recent years due to its broad applicability in various computer vision and image processing tasks, such as style transfer \cite{zhu2017unpaired, liu2017unsupervised, huang2018multimodal, jiang2020tsit, dutta2022seeing}, semantic segmentation \cite{park2019semantic, guo2020gan, li2020simplified, liu2019few}, image inpainting \cite{zhao2020uctgan, song2018contextual} and image enhancement \cite{chen2018deep}. To enforce structural preservation during the translation process, most recent GAN-based I2IT models use a cycle consistency mechanism \cite{zhu2017unpaired}, where an image is translated from the source domain (A) to the target domain (B) and then back from domain B to domain A during training, and a similarity loss is measured between the source image and the reconstructed one. This cycle consistency mechanism allows the network to learn the translation in an unsupervised manner. Unfortunately, it has encountered a discernible \color{purple} slowdown \color{black} in progress during the past few years. \dani{see my earlier comment about this, I don't think this statement is necessarily true, but it's also not necessary for our story}

\dani{I think the following should be shortened a bit. The paragraph is too long, and there are too many works and we can't discuss all of them at the level of a sentence or two per work. So need to define different groups of approaches, say generally what each group does, and cite a few representative works. Try to focus on works that could be viewed as I2I, and not just any kind of editing. For example the blended diffusion and GLIDE we can probably do without. On the other hand, I'd mention instruct pix2pix, because some I2I translations can be done with it.}
Following recent advancements in diffusion-based image synthesis quality, various models have been utilized for diffusion-based image manipulation tasks. SDEdit \cite{meng2021sdedit} first adds noise to the source image, alongside with editing guidance, and then denoises it using a diffusion process conditioned on the desired edit. Pix-to-pix zero \cite{parmar2023zero} suggests inverting the image to a seed using $\DDIM_\mathrm{inv}$ and then denoises it along a pre-calculated edit direction alongside a cross-attention mechanism, serving as a reference for the input image structure. Prompt-to-prompt \cite{hertz2022prompt} uses cross attention of the source image with values corresponding to edited text to retain structure, while enabling editing via changes in the prompt.  Imagic \cite{kawar2023imagic} allows non-rigid manipulations by first optimizing the target-related \edit{embedding} $e_{tgt}$ to get $e_{opt}$, 
\dani{What is $e$, is it an image, a latent?}
then fine-tuning the generative model to reconstruct the input image using $e_{opt}$ and finally interpolating between $e_{tgt}$ and $e_{opt}$ to generate the final editing result using the fine-tuned model. 
\dani{Should also cite the plug-and-play diffusion features paper here}
Another family of image-editing methods suggest using user-provided masks while keeping the rest of the image intact (\cite{avrahami2022blended, nichol2021glide}). \dani{Can omit the local mask-based methods.} 
Some papers have suggested different methods to control and optimize the diffusion process of a given pretrained model.
ControlNET \cite{zhang2023adding} presents a method to finetune a pretrained diffusion model while adding a spatial conditioning to control the structural semantics of the synthesized image. 
\dani{We should discuss SeedSelect, as we are doing something similar, but it's a separate paragraph, not related to I2I}
In SeedSelect \cite{samuel2023all} the authors present a way to synthesize concepts from the ``long-tail'' of the data distribution by carefully selecting suitable generation seeds in the noise space. In this study, we propose a series of optimization steps along the sampling trajectory. This approach aligns with previous research in which optimization along the trajectory has been explored. In pix2pix-zero \cite{parmar2023zero} optimization is utilized to enforce the adherence of the inverted noise maps generated by $DDIM_\mathrm{inv}$  \cite{song2020denoising}
to the statistical properties of uncorrelated, Gaussian white noise. In Null-text Inversion \cite{mokady2023null} the optimization employed for reconstructing the input image while facilitating the use of large guidance scale ($ > 1$). Subsequent studies, such as those presented in \cite{han2023improving, miyake2023negative} have further extended and enhanced the mechanisms originally proposed in \cite{mokady2023null} to achieve improved performance and computational efficiency.


In this work, we present the first diffusion-based I2IT model designed for global editing tasks, such as day-to-night or clear-to-fog transformations, using a single pre-trained Diffusion Model. Our model is capable of operating in complex automotive scenes, guided by textual input, and only requiring a few samples from the target domain. \par

==> sec/3_pre.tex <==
\subsection{Preliminaries}
\label{subsec:Preliminaries}
Diffusion Models (DMs) are generative models that synthesize images by iteratively denoising an initial randomly sampled noise $x_T \sim \mathcal{N}(0,I)$ in a controlled manner \cite{ho2020denoising}. We refer to the inital noisy image $x_T$ as the diffusion seed. Conditional DMs are diffusion models trained to generate images guided by some input control signal $c$. We denote by $\epsilon_t$ the noise predicted by the denoiser at timestamp $t$, i.e., $\epsilon_t = \epsilon_\Theta(x_t, t, c)$. Text-to-image diffusion models typically use Classifier-Free Guidance~\cite{ho2022classifier}, a mechanism where a guidance scale $\omega$ is used to control the amount of influence of the consition $c$ on the final output:
\begin{equation}
\label{eq:cfg}
\epsilon_t = \epsilon_\Theta(x_t, t, c_\varnothing) + \omega\cdot(\epsilon_\Theta(x_t, t, c) - \epsilon_\Theta(x_t, t, c_\varnothing)) 
\end{equation}
where $c_\varnothing$ denotes the representation of a null-text (``'') embedding.

The term $\DDIM_\mathrm{sam}$ \cite{song2020denoising} refers to a method of synthesising an image from a seed using a pre-trained diffusion model, with fewer denoising steps. A deterministic version of $\DDIM_\mathrm{sam}$  is shown below:
%
\begin{equation}
\label{eq:ddimSamp}
x_{t-1} = \sqrt{\alpha_{t-1}}\cdot pred_{x_0} + \sqrt{1-\alpha_{t-1}}\cdot\epsilon_t\cdot{x_t}
\end{equation}
%
where
\begin{equation}
\label{eq:predx0}
pred_{x_0} = \frac{x_t -\sqrt{1-\alpha_t}\cdot \epsilon_t\cdot{x_t}}{\sqrt{\alpha_t}}
\end{equation}
%
with $x_t$ a noisy sample at time $t$ and $\alpha_t$ being hyperparameter of the diffusion schedule defined per timestamp. In this paper, we adopt the DDIM reverse process (denoted $\DDIM_\mathrm{inv}$ ) to find a noise map $x_T$ that corresponds to the input image $x_0$. A deterministic version of this process can be formulated as:

\begin{equation}
\label{eq:dir_xt}
x_{t+1} = \sqrt{\alpha_{t+1}}\cdot pred_{x_0} + \sqrt{1-\alpha_{t+1}}\cdot\epsilon_t\cdot{x_t}
\end{equation}

Latent Diffusion Models (LDMs) \cite{rombach2022high} are DMs applied within a latent space of powerful pretrained autoencoders rather than directly on the image pixel space. In this paper we adopt Stable Diffusion \cite{rombach2022high} which encodes an input image $x_0 \in \mathcal{R}^{X\times X\times 3}$ to a latent representation $z_0\in \mathcal{R}^{S \times S \times 4}$.

==> sec/7_conc_1.tex <==
\section{Conclusions}
\label{sec:conc}

\dani{Given the new discussion section, this conclusions section is almost unnecessary, at the very least it could be shortened a lot.}
\Or{Maybe we can remove it all. Let's discuss it today at the meeting.}
We propose a novel I2IT method called S2ST. Our method performs image translation of complex (e.g., automotive) scenes, guided by a simple textual prompt and a few samples representing the target domain. To that end, we invert the source image to the seed space using $\DDIM_\mathrm{inv}$, then translate that source-related seed to a target-related one using an iterative optimization process we call Seed Translation (ST). Finally, we further enhance the content preservation in the generated image along the iterative sampling trajectory, defined by $\DDIM_\mathrm{sam}$ mechanism, in a process we call Trajectory Optimization (TO). \par

We compared our approach to different GAN-based and Diffusion based translation methods, showing superior performance int term of appearance in the target domain, while preserving the content of the source image. \par
Our method excels in generating localized effects that take into account the image's semantics, in addition to global translations that are not strictly dependent on image semantics. For instance, it effectively illuminates a car's lights while simultaneously dimming overall lighting during the transition from day to night, and adjusts shadows and reflections to align with the new lighting conditions.
\par
Moreover, contrary to typical GAN-based I2IT methods, our approach handles diverse domains (source and target) without requiring the training of a task-specific network for each domain pair.

==> sec/992_formatting.tex <==

\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/993_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
